From Historical Patches to Repair Plans: Outcome-Conditioned Reasoning for Repository-Level Program Repair

Repository-level automated program repair (APR) requires long-horizon reasoning over interdependent decisions. However, most LLM-based approaches reconstruct repair reasoning independently for each issue, failing to reuse successful patterns from prior repairs, even though real-world repositories contain many related issues with shared structure or constraints. Existing methods typically rely on forward exploration, which operates under outcome uncertainty, incurs substantial inference-time overhead, and can drift from the final correct patch. We propose Conditional Reasoning Distillation (ConRAD), which leverages in-repository resolved issues by reconstructing repair reasoning backward from verified patches and distilling outcome-consistent, stage-wise repair reasoning plans. Injected at inference time, these plans guide fault localization and patch generation, replacing open-ended exploration with constrained inference without fine-tuning or search. On SWE-Bench Lite, ConRAD improves Pass@1 by 10.4\% (GPT-4o), 8.6\% (DeepSeek-V3), and 10.3\% (GPT-5), demonstrating a scalable inference-time alternative to forward exploration for long-horizon APR.

==> rq2.tex <==

% \subsection{\peter{this RQ is the relationship of window size vs the bias, we don't know if limiting helps yet}RQ2: Does limiting context window help reduce the bias towards order?}
\subsection{RQ2: Does limiting context window help reduce the bias towards order?}

\phead{Motivation.}
In RQ1, we identified order bias in the sequence in which methods are presented in the zero-shot prompt. %However, it remains unclear whether smaller context windows can mitigate this bias. 
% \peter{remove this sentence - we don't know if the bias is really related to the context YET}To address this, we investigate whether a divide-and-conquer approach, where the input sequence is split into smaller contexts and each subset is reasoned individually, can reduce this bias. 
% \peter{I added it back}
We hypothesize that a larger context window might amplify the bias toward method order, as the LLM processes all methods simultaneously and may weigh their order more heavily when generating responses.
% \peter{revise based on above}Our goal is to understand how this approach impacts model performance, particularly in tasks where sequence length and order are critical, such as fault localization, program repair, and other software engineering tasks that require reasoning over code order.
In this RQ, we investigate how the context window influences order bias. Specifically, we examine how segmenting the input sequence into smaller independent segments affects LLM's performance in software engineering tasks, such as fault localization, where both context size and order play a crucial role in reasoning.
% \peter{the general idea is, when everythig is in one context, the LLM just looks at everything and the decision/response might be affected by the order the info is presented. Therefore, we want to study splitting the list into smaller context and study if this is true}n
% In RQ1, we found that the method order in the prompt significantly impacted the fault localization performance. This leads us to inquire whether the size of LLM's context windows correlates with the bias toward the order. ~\djk{Why we study context window is not entirely clear} Namely, would a large context window that takes all the methods in one prompt be more biased toward the method order? Our hypothesis is that a larger context window might amplify the bias toward method order, as the LLM processes all methods simultaneously and may weigh their order more heavily when generating responses.
% Hence, we in this RQ, we explore the relationship between context window size and the observed bias. 

%Specifically, we examine if dividing the information into smaller segments or reducing the context size can mitigate this bias. In this RQ, we explore the relationship between context window size and the observed bias, investigating whether presenting all information in a single large context versus splitting it into smaller segments affects the model's reasoning and fault localization outcomes.

% We examine the impact of splitting the context and providing information incrementally, aiming to understand whether the order still has an effect when the context window is smaller.

\phead{Approach.}
We investigate whether a divide-and-conquer approach, where the input sequence is split into smaller contexts and each subset is reasoned individually, can reduce this bias. We divide an ordered list of \( N \) methods, \( M=\{m_1, m_2, \dots, m_N\} \), into \( \max(\lceil N / S \rceil, 1) \) contiguous segments. Each segment \( M_i \subseteq M \) (for \( i = \{1, 2, \dots, J\} \)) contains up to \( S \) methods, ensuring \( |M_i| \leq S \). If \( S > N \), the entire list \( M \) forms a single segment (\( J = 1 \)). For this study, we experiment with five segment sizes \( S \in \{10, 20, 30, 40, 50\} \). In each segment  \( M_i \), the model ranks the Top-K suspicious methods \( R_i \), and the results \( R_i \) are summarized into \( G_i \). For the subsequent segment \( S_{i+1} \), the prompt includes both the \( M_{i+1} \) and the contextual information from \( G_i \). This iterative context-passing approach allows the model to re-rank methods based on combined information from previous segments. By incrementally varying the segment size (\(S\)), we analyze how the context window impacts order bias in fault localization. Specifically, we compare performance across two extreme ordering sequences: \perf (\(\tau = 1\)) and \worst (\(\tau = -1\)) (defined in RQ1) to assess whether the iterative context-passing effectively mitigates order bias, improving reliability across diverse ordering sequences.



% We divide an ordered list of \( N \) methods \( M = \{m_1, m_2, \dots, m_N\} \), which are covered by a failing test, into \( \max(\lceil N / S \rceil, 1) \) segments, each of size \( S \) or less. If the segment size \( S \) is greater than \( N \), the entire list \( M \) is treated as a single segment. We experiment with five segment sizes \( S \in \{10, 20, 30, 40, 50\} \). Each segment \( S_i \) contains methods \( M_i \subseteq M \), where \( |M_i| \leq S \).
% The model ranks the Top-K suspicious methods \( R_i \) from \( M_i \), and the results \( R_i \) are summarized into \( G_i \). For the next segment \( S_{i+1} \), the prompt includes \( M_{i+1} \) and \( G_i \), and the model re-ranks based on the combined information.
% In this iterative context passing, information from each segment are carried forward to the analysis in subsequent chunks. By incrementally adjusting the segment size (\(S\)), we analyze how the context window impacts order bias in fault localization. Specifically, we apply both \perf and \worst orders across varying segment sizes to observe if their performance converges as the segment size decreases, indicating a reduction in order bias as the segment size decreases. We consider two types of orders for ordering the methods within the segments: \perf (\(\tau = 1\)) and \worst (\(\tau = -1\)), as described in RQ1.

\phead{Results.} \textbf{\textit{The size of the context window impacts fault localization results, with larger context windows exhibiting a stronger order bias.}} Table~\ref{tab:split_comparison} presents the Top-K scores across different context segments for \perf and \worst. When the context is provided in larger segments (e.g., segment size 50), the model detects 278 bugs (55.5\%) in Top-1 with the \perf, while the \worst identifies only 170 bugs (33.9\%), around 22\% fewer bugs than the \perf. The large difference in Top-1 shows a significant order bias towards the order of the input method list. This is also evident in the Top 3, 5, and 10. For example, in the Top-10, the Perfect ranking reaches 408 (81.4\%) compared to 292 (58.3\%) for the Worst ranking, detecting around 23\% more bugs. 

As the segment size decreases, the difference between the \perf and \worst becomes smaller across all Top-K. For a segment size of 40, the model detects approximately 54\% of bugs in Top-1 with the \perf, which is 20\% more than the 34\% bugs detected with the \worst ranking. This pattern holds for Top-3, Top-5, and Top-10 as well. At a segment size of 30, the difference in Top-1 narrows further to 17\%, with \perf identifying 51\% of bugs compared to 34\% for \worst. When the segment size is reduced to 20, the \perf detects around 49\% of bugs in Top-1, while \worst detects 37\%, shrinking the difference to 12\%. This trend continues for Top-3, Top-5, and Top-10, where the performance gap between the two rankings becomes progressively smaller. 

At the smallest segment size of 10, there is nearly no difference in Top-1 (only a 1\% gap between \perf and \worst). Interestingly, for Top-3, Top-5, and Top-10, the model performs slightly better using the \worst compared to the \perf. These findings suggest that \textbf{\textit{as segment sizes decrease, the order bias toward the input order diminishes}}.

\rqboxc{As the context window size decreases, the order bias diminishes significantly, with the Top-1 gap between \perf and \worst rankings reducing from around 22\% at a segment size of 50 to just 1\% at a size of 10. Larger context windows tend to increase bias, whereas smaller context windows help reduce it.}

% \begin{table}[h!]
%     \caption{A comparison of fault localization performance across techniques and splits. The table highlights differences in Top-1, Top-3, Top-5, and Top-10 ranks for the techniques Perfect and Worst across various splits.}
%     \nakhla{Should we put percentage instead of numbers?}
%     \vspace{-0.3cm}
%     \centering
%     \label{tab:split_comparison}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|c|c|c|c|c}
%     \toprule
%         \textbf{Ranking} & \textbf{Split} & \textbf{Top-1} & \textbf{Top-3} & \textbf{Top-5} & \textbf{Top-10} \\ 
%     \midrule
%         Perfect & 10 & 217 & 295 & 313 & 338 \\ 
%         Worst   & 10 & 211 & 298 & 330 & 362 \\ 
%         \midrule
%         Perfect & 20 & 247 & 311 & 343 & 374 \\ 
%         Worst   & 20 & 186 & 265 & 288 & 335 \\ 
%         \midrule
%         Perfect & 30 & 261 & 326 & 347 & 382 \\ 
%         Worst   & 30 & 175 & 236 & 266 & 309 \\ 
%         \midrule
%         Perfect & 40 & 270 & 328 & 347 & 390 \\ 
%         Worst   & 40 & 171 & 223 & 249 & 284 \\ 
%         \midrule
%         Perfect & 50 & 278 & 338 & 368 & 408 \\ 
%         Worst   & 50 & 170 & 224 & 248 & 292 \\ 
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{-0.4cm}
% \end{table}


\begin{table}
    % \vspace{-0.3cm}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|c|c|c|c|c}
    \toprule
        \textbf{Ordering} & \textbf{Seg. Size} & \textbf{Top-1} & \textbf{Top-3} & \textbf{Top-5} & \textbf{Top-10} \\ 
    \midrule
        Perfect & 10 & 217 (43.3\%) & 295 (58.9\%) & 313 (62.5\%) & 338 (67.5\%) \\
        Worst & 10 & 211 (42.1\%) & 298 (59.5\%) & 330 (65.9\%) & 362 (72.3\%) \\
        \midrule
        Perfect & 20 & 247 (49.3\%) & 311 (62.1\%) & 343 (68.5\%) & 374 (74.7\%) \\
        Worst & 20 & 186 (37.1\%) & 265 (52.9\%) & 288 (57.5\%) & 335 (66.9\%) \\
        \midrule
        Perfect & 30 & 261 (52.1\%) & 326 (65.1\%) & 347 (69.3\%) & 382 (76.2\%) \\
        Worst & 30 & 175 (34.9\%) & 236 (47.1\%) & 266 (53.1\%) & 309 (61.7\%) \\
        \midrule
        Perfect & 40 & 270 (53.9\%) & 328 (65.5\%) & 347 (69.3\%) & 390 (77.8\%) \\
        Worst & 40 & 171 (34.1\%) & 223 (44.5\%) & 249 (49.7\%) & 284 (56.7\%) \\
        \midrule
        Perfect & 50 & 278 (55.5\%) & 338 (67.5\%) & 368 (73.5\%) & 408 (81.4\%) \\
        Worst & 50 & 170 (33.9\%) & 224 (44.7\%) & 248 (49.5\%) & 292 (58.3\%) \\

    \bottomrule
    \end{tabular}
    }
    \caption{A comparison of fault localization performance across techniques and segments. The table shows bugs detected in the Top-1, Top-3, Top-5, and Top-10 positions using \perf and \worst orders across various segments.}
    % ~\djk{make the table flow relative to text.}
    \vspace{-0.3cm}
    \label{tab:split_comparison}
\end{table}


==> rq3.tex <==

\subsection{RQ3: How do different ordering strategies influence fault localization performance?}
\label{rq3:section}
% \sw{How are methods typically ordered in SOTA FL approaches. I saw some FL approaches order method based on suspiciousness score.}\sw{ok, investigate tin RQ3}.
\phead{Motivation.} We find that LLMs may have order biases toward \perf when investigating a list of methods for FL. However, in practice, such ground truth ordering is unknown. Hence, in this RQ, we investigate whether ordering methods based on the static or dynamic nature of the code or using existing FL techniques can help LLMs achieve better FL results.

%Our previous research questions (RQs) established that the code order of input significantly impacts fault localization performance. Additionally, we found that placing relevant code information, such as ground truth methods, at the top of the input enhances results. However, in real-world scenarios, achieving the perfect order of code elements is often not possible. In these cases, rankings may need to rely on prior fault localization techniques or established metrics. 
% We found earlier that LLM may show bias towards the beginning of the code sequence when reasoning over a long sequence of methods. For example, using \perf resulted in the highest accuracy, and accuracy decreases as the order deviates from \perf. 



% We find that LLMs may have order biases toward \perf when investigating a list of methods for fault localization. However, in practice, such ground truth ordering is unknown. 
% Hence, in this RQ, we investigate whether we can leverage traditional fault localization techniques to order the methods and help large language models (LLMs) achieve better fault localization results. %This study aims to provide insights into the effectiveness of these rankings in real-world development tasks.


% \peter{rewrite. First say we try two families of approaches 1) traditional metrics and code-aware ordering 2) FL techniques. Their pros and cons. Then, introduce each technique.}


\phead{Approach.} We explore four types of ordering: (1) \textit{Statistical-based} and (2) \textit{Learning-based}, which are directly derived from FL techniques, and (3) \textit{Metric-based} and (4) \textit{Structure-based}, which are grounded in static code features and not specifically tied to FL. The first two approaches leverage dynamic execution data or advanced models trained on FL tasks, making them more targeted for identifying faults. In contrast, the latter two approaches are agnostic to FL techniques. Hence, they may lack the specificity needed for accurately identifying faults, as they do not directly utilize FL data. By integrating ordering strategies with the rich contextual information in the prompt template (see Figure~\ref{fig:prompt_example}), including test code, stack traces, and coverage data, we aim to strengthen LLMs' reasoning about the most relevant areas of the program, ultimately improving fault localization.

% Our findings reveal that while more complex fault localization metrics (e.g., learning-based approaches) may underperform in certain scenarios, they provide critical insights that justify the separation of these categories.

% We use (3) \textit{Statistical-based}, which relies on dynamic execution data; and (4) \textit{Learning-based}, which combines static and dynamic information. 

% By integrating ordering strategies with the rich contextual information in the prompt template (see Figure~\ref{fig:prompt_example}), including test code, stack traces, and coverage data, we aim to strengthen LLMs' reasoning about the most relevant areas of the program, ultimately improving fault localization.

% Our findings reveal that while more complex fault localization metrics (e.g., learning-based approaches) may underperform in certain scenarios, they provide critical insights that justify the separation of these categories.

For \textit{Metric-based} ordering, we use \textit{Lines of Code (LOC)}, ranking methods in descending order of their lines of code. Longer methods are often more complex and fault-prone~\cite{herraiz2010beyond}, making LOC a simple yet effective heuristic for prioritization. For \textit{Structure-based} ordering, we consider the structure of the call graph associated with each failing test. Specifically, we use \textit{Call Graph\textsubscript{DFS}}, which prioritizes deeper methods by traversing the call graph using depth-first search (DFS), and \textit{Call Graph\textsubscript{BFS}}, which highlights immediate dependencies by traversing the call graph using breadth-first search (BFS). By explicitly encoding dependency relationships, we evaluate whether these structural insights can help LLMs reason about fault propagation within the program and improve fault localization.

\textit{Statistical-based} ordering relies on dynamic execution data. For this, we use \textit{Ochiai}, which prioritize methods most likely to contain faults, offering insights beyond static metrics or structural heuristics. \textit{Ochiai} is a lightweight unsupervised Spectrum-Based Fault Localization (SBFL) technique~\cite{sasaki2020sbfl} based on the intuition that methods covered by more failing tests and fewer passing tests are considered more suspicious (e.g., faulty). Its suspiciousness score is computed as:

{\small
\begin{equation*}
Ochiai(a_{ef}, a_{nf}, a_{ep}) = \frac{a_{ef}}{\sqrt{(a_{ef} + a_{nf}) \times (a_{ef} + a_{ep})}}
\end{equation*}
}

Here, \(a_{ef}\), \(a_{nf}\), and \(a_{ep}\) denote the number of failed and passed test cases that execute or do not execute a code statement. Scores range from 0 to 1, with higher values indicating higher fault likelihood. We order methods by aggregating their statement-level scores. 

Finally, for \textit{Learning-based} ordering, we use \textit{DepGraph}, which is the state-of-the-art supervised FL technique based on graph neural network~\cite{depgraph} that transforms the rich static and dynamic code information into a graph structure. It trains a graph neural network to rank faulty methods by analyzing structural code dependencies and code change history (see Appendix \ref{depgraph_appendix}).

% ~\djk{add details about depgrap. add why it has rich info}.


% We study two traditional FL techniques—\textit{Ochiai} and \textit{DepGraph} to derive method rankings based on suspiciousness scores. These techniques prioritize methods most likely to contain faults, offering insights beyond static metrics or structural heuristics. \textit{Ochiai} is a lightweight unsupervised Spectrum-Based Fault Localization (SBFL) technique~\cite{sasaki2020sbfl} based on the intuition that methods covered by more failing tests and fewer passing tests are considered more suspicious. Its suspiciousness score is computed as:

% {\small
% \begin{equation*}
% Ochiai(a_{ef}, a_{nf}, a_{ep}) = \frac{a_{ef}}{\sqrt{(a_{ef} + a_{nf}) \times (a_{ef} + a_{ep})}}
% \end{equation*}
% }

% Here, \(a_{ef}\), \(a_{nf}\), and \(a_{ep}\) denote the number of failed and passed test cases that execute or do not execute a code statement. Scores range from 0 to 1, with higher values indicating higher fault likelihood. We order methods by aggregating their statement-level scores. \textit{DepGraph} is the state-of-the-art supervised FL technique based on graph neural network~\cite{depgraph} that transforms the dynamic coverage information in a graph structure. 
% It trains a graph neural network %network-based algorithm 
% to rank suspicious methods by analyzing structural code dependencies and code change history. 






% \phead{Approach.} To explore whether ordering based on traditional fault localization techniques improves LLM fault localization, we investigate four approaches:  (1) \textit{Traditional Metrics and Code-Aware Ordering} and (2) \textit{Fault Localization (FL) Techniques and Rankings}. Traditional metrics and code-aware ordering use static properties of the code, such as lines of code or call graph structure, to prioritize methods. While these approaches are lightweight and widely applicable, they may miss insights specific to certain faults. In contrast, fault localization (FL) techniques generate rankings based based on test coverage and failure information, providing fault-specific prioritization but requiring additional runtime data or model training.


% Traditional metrics and code-aware ordering use static properties of the code, such as lines of code or call graph structure, to prioritize methods. While these approaches are lightweight and widely applicable, static properties lack dynamic insights from code execution. In contrast, fault localization (FL) techniques generate rankings based based on test coverage and failure information, providing fault-specific prioritization but requiring additional runtime data or model training.

% ~\djk{Make it clear the only diff between codeaware and Traditional SBFL is ordering. Moreover, the way it's written make it sounds like codeaware does not use any execution info.}


% ~\djk{Idk why it should be called code-aware, since everything is the same, but only diff is order. Based on RQ1, there is orer bias, not sure how these code aware metrics add more code aware metrics...}


% For traditional metrics-based ordering, we use \textit{Lines of Code (LOC)}, where methods are ranked in descending order of their lines of code. Longer methods are often more complex and fault-prone~\cite{ herraiz2010beyond}, making LOC a simple yet effective heuristic for prioritization. For code-aware ordering, we consider the structure of the call graph associated with each failing test. Specifically, we use \textit{Call Graph\textsubscript{DFS}}, which prioritizes deeper methods by traversing the call graph using depth-first search (DFS), and \textit{Call Graph\textsubscript{BFS}}, which highlights immediate dependencies by traversing the call graph using breadth-first search (BFS). \peter{what is the intuition? the code follows a sequential order, may be closer to what LLM's training}


% We study two traditional FL techniques—\textit{Ochiai} and \textit{DepGraph} to derive method rankings based on suspiciousness scores. These techniques prioritize methods most likely to contain faults, offering insights beyond static metrics or structural heuristics. \textit{Ochiai} is a lightweight unsupervised Spectrum-Based Fault Localization (SBFL) technique~\cite{sasaki2020sbfl} based on the intuition that methods covered by more failing tests and fewer passing tests are considered more suspicious. Its suspiciousness score is computed as:

% {\small
% \begin{equation*}
% Ochiai(a_{ef}, a_{nf}, a_{ep}) = \frac{a_{ef}}{\sqrt{(a_{ef} + a_{nf}) \times (a_{ef} + a_{ep})}}
% \end{equation*}
% }

% Here, \(a_{ef}\), \(a_{nf}\), and \(a_{ep}\) denote the number of failed and passed test cases that execute or do not execute a code statement. Scores range from 0 to 1, with higher values indicating higher fault likelihood. We order methods by aggregating their statement-level scores. \textit{DepGraph} is the state-of-the-art supervised FL technique based on graph neural network~\cite{depgraph} that transforms the dynamic coverage information in a graph structure. 
% It trains a graph neural network %network-based algorithm 
% to rank suspicious methods by analyzing structural code dependencies and code change history. 


%DepGraph, which is the state-of-the-art supervised FL technique, produces a sorted list of methods by their fault likelihood, using which we order the methods.

% \uhead{Ochiai} is a well-known Spectrum-based-fault-localization (SBFL) technique~\cite{sasaki2020sbfl}. It is a statics-based approach where a method covered by more failing tests and less passing tests is considered more suspicious. It is very lightweight and has been used in many prior researches~\cite{li2019deepfl, vacheret2024boosting}. We first gather the suspiciousness ranking for each of the project's bugs using the algorithm, and then we sort the covered methods based on the scores in descending order. Ochiai is defined as: 

% {\small
% \begin{equation*}
% Ochiai(a_{ef}, a_{nf}, a_{ep}) = \frac{a_{ef}}{\sqrt{(a_{ef} + a_{nf}) \times (a_{ef} + a_{ep})}}
% \end{equation*}
% }


% where \(a_{ef}\) is the number of failed test cases that execute a statement, \(a_{nf}\) is the number of failed test cases that do not execute the statement, and \(a_{ep}\) is the number of passed test cases that execute the statement. The result of Ochiai is a value between 0 and 1, with higher values indicating a higher likelihood that a particular statement is faulty. We then aggregate the scores for every statement in a method to get the method-level score.


% \uhead{DepGraph} is a recent fault localization technique based on graph neural networks~\cite{depgraph}. It ranks methods by considering structural code dependencies and the history of code changes. DepGraph demonstrates impressive performance compared to other fault localization techniques in the field. We apply this technique to each bug and compile the suspicious rankings to sort the covered methods in descending order.

% \begin{table}[h!]
%     \caption{Comparison of fault localization performance using different metrics based ordering.}
%     \vspace{-0.3cm}
%     \centering
%     \label{tab:technique_comparison}
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l|c|c|c|c}
%     \toprule
%         \textbf{Technique} & \textbf{Top-1} & \textbf{Top-3} & \textbf{Top-5} & \textbf{Top-10} \\ 
%     \midrule
%         DepGraph        & 242.0 & 338.0 & 386.0 & 419.0 \\ 
%         \midrule
%         CallGraph\textsubscript{BFS}  & 175.0 & 252.0 & 294.0 & 343.0 \\ 
%         \midrule
%         CallGraph\textsubscript{DFS}  & 173.0 & 253.0 & 305.0 & 351.0 \\ 
%         \midrule
%         Ochiai          & 164.0 & 252.0 & 293.0 & 342.0 \\ 
%         \midrule
%         LOC             & 163.0 & 256.0 & 289.0 & 351.0 \\ 
%     \bottomrule
%     \end{tabular}
%     }
%     \vspace{-0.4cm}
% \end{table}

\begin{table}
    % \vspace{-0.3cm}
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ll|c|c|c|c}
    \toprule
       \multicolumn{2}{l|}{ \textbf{Technique} }& \textbf{Top-1} & \textbf{Top-3} & \textbf{Top-5} & \textbf{Top-10} \\ 
       \midrule
        \multicolumn{2}{l|}{\textit{\underline{Learning-based}}} & & & & \\
         & {DepGraph} & 242.0 (48.3\%) & 338.0 (67.5\%) & 386.0 (77.0\%) & 419.0 (83.6\%) \\
        \midrule
        \multicolumn{2}{l|}{\textit{\underline{Structure-based}}} & & & & \\
        & {CallGraph\textsubscript{BFS}} & 175.0 (34.9\%) & 252.0 (50.3\%) & 294.0 (58.7\%) & 343.0 (68.5\%) \\
        & {CallGraph\textsubscript{DFS}} & 173.0 (34.5\%) & 253.0 (50.5\%) & 305.0 (60.9\%) & 351.0 (70.1\%) \\
        \midrule
        \multicolumn{2}{l|}{\textit{\underline{Statistical-based}}} & & & & \\
        & {Ochiai} & 164.0 (32.7\%) & 252.0 (50.3\%) & 293.0 (58.5\%) & 342.0 (68.3\%) \\
        \midrule
        \multicolumn{2}{l|}{\textit{\underline{Metric-based}}} & & & & \\
        & {LOC} & 163.0 (32.5\%) & 256.0 (51.1\%) & 289.0 (57.7\%) & 351.0 (70.1\%) \\

    \bottomrule
    \end{tabular}
    }
    \caption{Comparison of fault localization performance using different ordering strategies with the percentage of bugs found across 501 total faults.}
    \label{tab:technique_comparison}
    \vspace{-0.3cm}
\end{table}


\phead{Results.}
\textbf{\textit{The choice of ordering strategy is critical in LLM's ability to localize faults, with FL-derived ordering using \textit{DepGraph} detecting almost 13.4\% more faults in Top-1 compared to the next highest Top-1, achieved by \textit{Call Graph\textsubscript{BFS}}}}.  Table~\ref{tab:technique_comparison} highlights the model's effectiveness across different ordering strategies. \textit{DepGraph} identifies 13.4\%  more faults in the Top-1 rank. We see similar trends among other Top-K, where \textit{DepGraph} identifies 16\% more faults in Top-3, 16.1\% in Top-5, and 13.5\% in Top-10. This performance difference is expected, as \textit{DepGraph} excels at ranking faulty methods higher on the list through its advanced fault localization capabilities. The additional faults localized by \textit{DepGraph} across all Top-K ranks reinforce our earlier observation that \textbf{\textit{improved ordering strategies enable the model to prioritize the most suspicious methods earlier}}. 

Despite the importance of order bias, actual FL methods like \textit{DepGraph} provide significantly better fault localization than techniques that do not use LLMs. For instance, \textit{DepGraph}'s Top-K results are higher: 299 (Top-1), 382 (Top-3), 415 (Top-5), and 449 (Top-10) compared to the results from LLM-based methods (see Appendix \ref{appendix:traditiona_approach_perf}). The results suggest that \textit{\textbf{while LLMs can help with tasks such as ranking faulty methods, domain-specific methods (like DepGraph) are still superior for accurate results}}. 

% \vspace{-14mm}

Interestingly, \textit{Ochiai} reveals an interesting trend: \textbf{\textit{leveraging simple statistical metrics can enable LLMs to improve fault localization by better prioritizing fault-prone methods}}. This finding indicates that while \textit{Ochiai}, a simpler \textit{Statistical-based} method, does not match the accuracy of \textit{DepGraph}, it can still effectively assist in fault localization, particularly when computational efficiency or simplicity is a priority. \textit{Ochiai} offers LLMs a simpler way to rank methods based on test outcomes, which aligns well with their ability to process observable patterns. In contrast, \textit{DepGraph} relies on complex code structures like dependencies and execution traces, which require a \textbf{\textit{deeper understanding that LLMs may not possess, making it harder for them to reason effectively}}.

\textbf{\textit{Simple static-based ordering strategies can match or even outperformance more complex FL-derived ordering across all Top-K ranks.}} For instance, \textit{CallGraph\textsubscript{BFS}}, which prioritizes methods closer to failing tests, identifies 175 bugs in Top-1 (34.9\%), slightly outperforming \textit{CallGraph\textsubscript{DFS}} with 173 bugs (34.5\%) and achieving a higher Top-1 accuracy (32.7\%) compared to the more complex \textit{Statistical-based} ordering. A similar trend is observed across the remaining Top-K ranks, where \textit{CallGraph\textsubscript{DFS}} either matches or slightly outperforms \textit{Statistical-based} ordering, with differences ranging from 0\% to 0.02\%. Additionally, when comparing \textit{Statistical-based} ordering with \textit{Metric-based} methods, it shows comparable performance in Top-1 ($\Delta 0.2\%$) and Top-3 ($\Delta 0.8\%$), but outperforms in Top-5 ($\Delta 0.8\%$) and Top-10 accuracy ($\Delta 1.8\%$). This suggests that static methods, which are computationally less demanding, can still be effective for fault localization. Hence, these findings emphasize the practicality of \textbf{\textit{simpler static-based methods as viable alternatives to more complex FL techniques}}. 


\rqboxc{While ordering helps rank faults, LLMs struggle with complex relationships. Simpler static-based methods, like \textit{CallGraph\textsubscript{BFS}}, perform comparably to more complex \textit{Statistical-based} ordering like \textit{Ochiai} in fault localization. Our findings highlight the practicality of static-based methods as efficient alternatives to complex FL techniques, particularly in resource-constrained environments.}





% \textbf{\textit{Structural-based ordering strategies show comparable performance in fault localization across all Top-K where the percentage of bugs found in Top-1 lies in between around 32\% to 35\%.}} CallGraph\textsubscript{BFS}, which prioritizes methods closer to failing tests, identifies 175 bugs in Top-1 (34.9\%), marginally outperforming CallGraph\textsubscript{DFS} at 173 bugs (34.5\%). As we move to broader ranks, CallGraph\textsubscript{DFS} detects 351 bugs in Top-10 (70.1\%), slightly surpassing BFS’s 343 bugs (68.5\%). LOC, a simpler metric that orders methods by their complexity (measured by lines of code), performs consistently across ranks, starting with 163 bugs in Top-1 (32.5\%) and matching DFS at Top-10 with 351 bugs (70.1\%). These results indicate that while there are subtle differences in how these strategies prioritize methods, they achieve relatively similar outcomes in localizing faults across larger ranks, highlighting their utility as practical alternatives to more advanced techniques like DepGraph.

% \peter{need a discussion on the how to choose the ordering: smaller context vs static vs depgraph}


% \noindent\textbf{\textit{Traversal-based strategies also show differences in results, highlighting the impact of how methods are prioritized.}} CallGraph\_BFS detects 175 faults at Top-1, or about 12 more than Ochiai, and achieves 343 bugs at Top-10, matching Ochiai’s performance. On the other hand, CallGraph\_DFS starts with a slightly lower Top-1 score of 173 faults, but by Top-10, it edges past BFS, detecting 351 faults—8 more bugs localized. This suggests that BFS’s focus on proximity to failing tests benefits earlier ranks, while DFS’s exploration of deeper dependencies proves advantageous for broader ranks. Similarly, LOC, which orders methods by their lines of code, starts at the same level as Ochiai in Top-1 with 163 bugs but improves at higher ranks, tying with DFS at 351 bugs Top-10. These findings underscore the importance of designing thoughtful ordering strategies: DepGraph provides the most effective rankings, but even lightweight methods like Ochiai or traversal-based strategies can perform competitively in broader contexts.

